A Control Architecture for Entanglement Generation Switches in Quantum Networks

Entanglement between quantum network nodes is often produced using intermediary devices - such as heralding stations - as a resource. When scaling quantum networks to many nodes, requiring a dedicated intermediary device for every pair of nodes introduces high costs. Here, we propose a cost-effective architecture to connect many quantum network nodes via a central quantum network hub called an Entanglement Generation Switch (EGS). The EGS allows multiple quantum nodes to be connected at a fixed resource cost, by sharing the resources needed to make entanglement. We propose an algorithm called the Rate Control Protocol (RCP) which moderates the level of competition for access to the hub's resources between sets of users. We proceed to prove a convergence theorem for rates yielded by the algorithm. To derive the algorithm we work in the framework of Network Utility Maximization (NUM) and make use of the theory of Lagrange multipliers and Lagrangian duality. Our EGS architecture lays the groundwork for developing control architectures compatible with other types of quantum network hubs as well as system models of greater complexity.

==> LongResultsSummary.tex <==
\begin{itemize}
    \item What: Theorem \ref{thm:CapReg}, characterizes the capacity region of the EGS, which is the maximal set of rates at which users can submit demands to the EGS such that the demands are served at the same rate which they are submitted (in other words the EGS is stabilized). Moreover, the theorem guarantees that when the Maximum Weight Scheduling policy (Definition \ref{def:MaxWeight}) for resource allocation is used by the EGS, then the switch is stabilized for any rate vector from within the capacity region. Implications: In the context of developing an algorithm to regulate the competition for EGS resources, the capacity region of the switch, which is guaranteed to be well-defined by the theorem, provides the constraints which should be used to define the set of arrival rate vectors admissible by the algorithm for regulating competition. Caveats/Extensions: If a different resource allocation scheduling policy is used, the capacity region remains unchanged, however, the subset of rate vectors from the capacity region that result in demands that can be served in a finite time under the selected scheduling policy may be reduced.
 
    
    \item What: We derive the Rate Control Protocol (RCP), an algorithm to regulate the rates at which pairs of users submit demands for bi-partite entanglement to the central switch of an EGS. Implications: The RCP outputs rate vectors that are optimal in the sense that they are guaranteed to make full use of the entanglement generation capacity of the EGS, satisfy the minimum rate requirements of all requesting user pairs, and not to cause any user to submit demands at rates exceeding their network node's capability to consume entanglement. Caveats/Extensions: The control algorithm can be straightforwardly extended to the context of multi-partite entanglement generation via an EGS by proper selection of an entanglement generation protocol, selection of resource modules, and generalization of a communication session to consist of multiple users in place of user pairs.
    
    \item Theorem: Convergence of the RCP: We prove (Theorem \ref{thm:ConvergenceThm}) that the sequence of arrival rate vectors output by the RCP converges to an optimum value. Implications: Therefore, when all requesting user pairs update their demand submission rates at the end of every time-slot to the value calculated by the RCP, the resulting rate vectors converge to an optimal solution. Caveats/Extensions: Convergence is guaranteed independently of the initial rate vector, thus the initial demand submission rates set by the user pairs do not affect the convergence. A caveat is that convergence to an optimum is only guaranteed when the step-size of the RCP is sufficiently small.\footnote{The precise step-size cutoff is specified in Theorem \ref{thm:ConvergenceThm}}
    
    \item 
    What: The tightness of the convergence ($\delta$) guaranteed by Theorem \ref{thm:ConvergenceThm} and the number of time slots ($\Delta \tau$) that the RCP must run before convergence is achieved, called the convergence time, depend on both the number of user pairs that submit demands for entanglement generation and the step-size used in the RCP. We illustrate with numerical simulations several possible values of $\delta$ and $\Delta \tau$ that can be achieved. Implications: It is possible to target decreasing values of $\delta$ or $\Delta \tau$ by tuning the step-size used in the RCP or the number of user pairs demanding entanglement generation. Caveats/Extensions: In the set of simulations performed a trade-off between the tightness of convergence and the convergence time was observed. Simulations were only performed for a setting where every user pair supplies a logarithmic utility function to the RCP. 
\end{itemize}
